Enumerating maximal cliques in link streams with durations

Link streams model interactions over time, and a clique in a link stream is defined as a set of nodes and a time interval such that all pairs of nodes in this set interact permanently during this time interval. This notion was introduced recently in the case where interactions are instantaneous. We generalize it to the case of interactions with durations and show that the instantaneous case actually is a particular case of the case with durations. We propose an algorithm to detect maximal cliques that improves our previous one for instantaneous link streams, and performs better than the state of the art algorithms in several cases of interest.

==> delta.tex <==
In this section, we show that there is an equivalence between the cliques defined in this paper and the $\Delta$-cliques defined in~\cite{viard2016computing}.
%\todo[inline]{Def $\Delta$-cliques}

%For a link stream $L=(T,V,E)$ with $|V|=n$ and $T=[\alpha, \omega]$, we define its density as $\delta(L)= \frac{2\cdot \sum_{(b,e,u,v)\in E} e- b}{n\cdot (n-1) \cdot (\omega - \alpha)}$.
%It is the probability, when one takes a time $t$ in $T$ at random and two nodes $u$ and $v$ in $V$ at random, that there exists a link $(b,e,u,v)$ in $E$ with $t$ in $[b,e]$. 
%A clique $(X, [b,e])$, $X\subseteq V$, $[b,e]\subseteq T$, is a substream of density $1$.

% L_\Delta
%\begin{figure}
	%\begin{center}
		%%\includegraphics{}
		%\caption{Stream transformation}
		%\label{fig:}
	%\end{center}
%\end{figure}


Given an instantaneous link stream $L=(T,V,E)$, $T=[\alpha, \omega]$, $E\subseteq T\times V\times V$, and a value $\Delta \in [0,\omega-\alpha]$, 
we define the link stream $L'_\Delta=(T_\Delta,V, E'_\Delta)$ such that $T_\Delta = [\alpha+\Delta, \omega]$ 
and $E'_\Delta = \{(t, t+\Delta,u,v) \cap T_\Delta: \exists (t,u,v)\in E \}$. 
In other words, any two nodes are linked together at time $t$ in $L_\Delta$ if and only if they are linked together in $L$ at a time $t' \in [t-\Delta,t]$.

Notice that $L'_\Delta$ is not simple:
there might be links $(b,e,u,v)$ and $(b',e',u,v)$ such that $[b,e]\cap [b',e']\ne\emptyset$. 
We define $L_\Delta=(T_\Delta, V, E_\Delta)$ as the simplification of $L'_\Delta$, 
obtained for instance by iteratively replacing overlapping links $(b,e,u,v)$ and $(b',e',u,v)$
by their union $(\min(b,b'),\max(e,e'),u,v)$.

        
% Then, we have $\delta_\Delta(L) = \delta(L_\Delta)$. Indeed, $\delta_\Delta(S)$ is the probability, when one takes a random time interval of duration $\Delta$ in $T$ and two random nodes $u$ and $v$ in $V$ that these two nodes are linked together at some time during this time interval. This is equivalent to taking a random time instant $t$ in $[\alpha+\demidelta, \omega-\demidelta]$ such that the two nodes are linked together at some time in $[t-\demidelta,t+\demidelta]$ in $S$. By definition of $S_\Delta$, this is equivalent to taking $t$ in $T_\Delta$ such that the two nodes are linked together at time $t$ in $S_\Delta$: if the nodes are linked together at some time in $[t-\demidelta,t+\demidelta]$ in $S$ then they are linked together at time instant $t$ in $S_\Delta$, and conversely. The probability that this occurs is nothing but the density of $S_\Delta$.      
        
%\todo[inline]{Densité ou cliques directement ?}     
        
Let us now show that there is an equivalence between $\Delta$-cliques in $L$ and cliques in $L_\Delta$.

We first define a bijective transformation between the $\Delta$-cliques of $L$ and
the cliques of $L_\Delta$.
Given a $\Delta$-clique $C=(X, [b,e])$ in $L$,
we associate it to the clique $C_\Delta = (X, [b+\Delta,e])$ in $L_\Delta$.
We will show below that this transformation indeed respects the clique structure,
as well as maximality.

%\todo[inline]{Définir time-maximal ci-dessous}
We say that a clique $(X,[b,e])$ is \emph{time-maximal} if there is no $[b',e'] \supset [b,e]$ such that $(X, [b',e'])$ is a clique.  

\begin{lemma}
  $C=(X, [b,e])$ is a time-maximal $\Delta$-clique in $L$ if and 
  only if $C_\Delta = (X, [b+\Delta,e])$ is a time-maximal clique in $L_\Delta$.
  \label{lem:time-max}
\end{lemma}
\begin{proof}
  Assume $C=(X, [b,e])$ is a time-maximal $\Delta$-clique in $L$.
This implies that for any $u,v\in X$ and any $t \in [b+\Delta, e]$,
there exists a time $t'\in [t-\Delta,t]$ such that $(t',u,v)\in E$.
This implies that $u$ and $v$ are linked at time $t$ in $L_\Delta$ and
therefore that $C_\Delta = (X, [b+\Delta,e])$ is a clique in $L_\Delta$.

Assume $C_\Delta$ is not time-maximal.
This means that there exists either a time $e'$, $e < e' < e+\Delta$ such that
$(X, [b+\Delta, e'])$ is a clique,
or a time $b'$, $b-\Delta < b' < b$ such that $(X, [b'+\Delta, e])$ is a clique
(notice that $b'$ (resp. $e'$) may not be the smallest value such that $(X, [b'+\Delta, e])$
(resp. $(X, [b+\Delta, e'])$) is a clique).
Assume there exists such a time $e'$.
This implies that for all $u,v\in X$,  and all times 
$t \in [e,e']$,
$u$ and $v$ are linked in $L_\Delta$ at time $t$
and therefore 
there exists a time $t' \in [t-\Delta, t]$ such that $(t',u,v) \in E$.
This in turns implies that $(X, [b, e'])$ is a $\Delta$-clique in $L$
and therefore that $C$ is not time-maximal, contradicting our initial assumption.
A similar argument can be used to show that there exists no $b'$ as described above,
and finally that $C_\Delta$ is time-maximal.

%\todo[inline]{Vrai qu'on peut utiliser le même argument pour $b'$ ?}

\medskip

Assume now that $C_\Delta = (X, [b+\Delta,e])$ is a time-maximal clique in $L_\Delta$.
This implies that for all $u,v\in X$ and all $t\in [b+\Delta,e]$,
there exists a $t'\in [t-\Delta, t]$ such that $(t',u,v) \in E$.
This implies that $C=(X,[b,e])$ is a $\Delta$-clique.

Assume $C$ is not time-maximal.
This means that there exists either a time $e'$, $e < e' < e+\Delta$ such that
$(X, [b, e'])$ is a $\Delta$-clique,
or a time $b'$, $b-\Delta < b' < b$ such that $(X, [b', e])$ is a $\Delta$-clique.
Assume there exists such a time $e'$.
This implies that for all $u,v\in X$ and for all $t\in [e,e']$,
there exists a time $t'$, $t-\Delta < t' < t$
such that $(t',u,v)\in E$.
This in turns implies that $u$ and $v$ are linked from $e$ to $e'$ in $L_\Delta$ and
that $(X, [b+\Delta,e'])$ is a clique,
therefore $C_\Delta$ is not time-maximal, contradicting our assumption.
A similar argument can be used to show that there exists no $b'$ as described above,
and finally that $C$ is time-maximal.

\end{proof}


We can now show that maximal $\Delta$-cliques in $L$ correspond to maximal
cliques in $L_\Delta$.

\begin{theorem}
  $C=(X, [b,e])$ is a maximal $\Delta$-clique in $L$ if and 
  only if $C_\Delta = (X, [b+\Delta,e])$ is a maximal clique in $L_\Delta$.
\end{theorem}
\begin{proof}
If $C$ is a maximal $\Delta$-clique,
we know from Lemma~\ref{lem:time-max} that $C_\Delta$ is a time-maximal
clique in $L_\Delta$.
Assume $C_\Delta$ is not maximal,
this means that there exists a vertex $v\in V\backslash X$ such that
${C_\Delta}v=(X\cup \{v\}, [b+\Delta, e])$ is a clique.  
${C_\Delta}v$ is time-maximal because $C_\Delta$ is time-maximal.
Therefore, from Lemma~\ref{lem:time-max},
$C_v = (X\cup \{v\}, [b,e])$ is a $\Delta$-clique,
which contradicts the assumption that $C$ is maximal.

A similar argument can be used to show that,
if  $C_\Delta = (X, [b+\Delta,e])$ is a maximal clique in $L_\Delta$,
then $C=(X, [b,e])$ is a maximal $\Delta$-clique in $L$,
which concludes the proof.
\end{proof}

Notice that the time complexity of the algorithm we propose here is slightly lower than the one of the algorithm presented in~\cite{viard2016computing}, which was in ${\cal O}(2^nn^3m^2 + 2^nn^2m^3)$.
Moreover, given an instantaneous link stream $L$ and a parameter $\Delta$,
computing $L_\Delta$ from $L$ can trivially be done in ${\cal O}(m^2)$ time
($m$ steps to add a duration of $\Delta$ to each link,
then ${\cal O}(m^2)$ steps to simplify the resulting link stream,
e.g. by iteratively replacing overlapping links by their union).
This means that computing maximal $\Delta$-cliques in an instantaneous link stream $L$
can be done more efficiently by computing maximal cliques in $L_\Delta$.

This is interesting, as in many cases of interest,
$n$ is small with respect to $m$ (notice that in link streams $m$ can be much
larger than $n^2$, 
contrary to what happens in graphs),
and the gain from a $m^3$ factor to a $m^2\log m$ factor is not negligible,
even in the face of a $2^n$ factor.



%\section{Experimentations}

%Dataset Thiers-Highschool. We build the link stream by grouping two links separated by 20 seconds or less, based on the resolution of the capture (cite Fournet, Barrat). i.e. $(b,e,u,v)\in E \implies \forall t\in [b,e], \exists (t',u,v)\in D s.t. t' \in [t-20, t+20]\cap [b,e]$.

%\question{Dataset NHK ?}

%\begin{figure}
%\missingfigure{Tailles + durées des cliques maximales}
%\label{fig:size-dur-cliques}
%\caption{Left: ... Right: ...}
%\end{figure}

%Ajouter des temps de calcul comparatifs au delta-cliques ?




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "algo"
%%% End:

